Network Estimation by Mixing: Adaptivity and More

Networks analysis has been commonly used to study the interactions between units of complex systems. One problem of particular interest is learning the network's underlying connection pattern given a single and noisy instantiation. While many methods have been proposed to address this problem in recent years, they usually assume that the true model belongs to a known class, which is not verifiable in most real-world applications. Consequently, network modeling based on these methods either suffers from model misspecification or relies on additional model selection procedures that are not well understood in theory and can potentially be unstable in practice. To address this difficulty, we propose a mixing strategy that leverages available arbitrary models to improve their individual performances. The proposed method is computationally efficient and almost tuning-free; thus, it can be used as an off-the-shelf method for network modeling. We show that the proposed method performs equally well as the oracle estimate when the true model is included as individual candidates. More importantly, the method remains robust and outperforms all current estimates even when the models are misspecified. Extensive simulation examples are used to verify the advantage of the proposed mixing method. Evaluation of link prediction performance on 385 real-world networks from six domains also demonstrates the universal competitiveness of the mixing method across multiple domains.

==> Theory.tex <==


We now present the theoretical support for the NNLS estimate. Let
\begin{eqnarray*}
\mathcal{L}=\text{span}\{\hat{P}^{(r)}(\Omega),1\le r\le m\}, \quad \mathcal{C}=\text{cone}\{\hat{P}^{(r)}(\Omega),1\le r\le m\}
\end{eqnarray*}
be the linear subspace and the cone generated by $\{\hat{P}^{(r)}(\Omega),1\le r\le m\}$, and $\Pi_\mathcal{L}$ and $\Pi_\mathcal{C}$ be the projections onto $\mathcal{L}$ and $\mathcal{C}$, respectively. Also, denote 
$$\|\hat{P}^{(r)}(\Omega)\|_\infty=\max_{(i,j)\in\Omega}|\hat{P}^{(r)}_{ij}|, \qquad \|P(\Omega)\|_\infty = \max_{(i,j)\in\Omega}P_{ij}.$$ 

\begin{thm}[Non-negative least square estimate, positive inter products]\label{thm:nnls}
Let $A$ be the adjacency matrix of a random network drawn from the inhomogeneous Erd\H{o}s-R\'{e}nyi model with probability matrix $P=\mathbb{E} A$. For a fixed $p\in(0,1)$, let $\Omega$ be the index set obtained by independently selecting elements of $[n]^2$ with probability $p$, and $\hat{A}$ be the matrix obtained from $A$ by setting entries of $A$ with indices in $\Omega$ to zero. Denote by $\hat{P}^{(r)}$, $1\le r \le m$, the estimates of $P$ obtained by applying the methods from $\mathcal{M}$ on $\hat{A}$ and let $\hat{P}$ be the NNLS estimate defined by \eqref{eq:nnls estimate} and assume that
\begin{equation}\label{eq:correlated assumption}
\delta  = \min_{1\le r,s\le m}\frac{\big\langle \hat{P}^{(r)}(\Omega),\hat{P}^{(s)}(\Omega) \big\rangle}{\|\hat{P}^{(r)}(\Omega)\|_F\cdot\|\hat{P}^{(s)}(\Omega)\|_F}>0.
\end{equation}
Then there exists a constant $C>0$ such that with high probability,
\begin{eqnarray}\label{eq:nnls bound}
\|\hat{P}(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F &\le& \|\Pi_\mathcal{C}\Pi_\mathcal{L} P(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F + C\delta^{-1/2}\varepsilon, 
\end{eqnarray} 
where $C>0$ is a constant and
\begin{eqnarray*}
\varepsilon = \max_{1\le r \le m}\frac{\|\hat{P}^{(r)}(\Omega)\|_\infty}{\|\hat{P}^{(r)}(\Omega)\|_F}\cdot\log m +(\|P(\Omega)\|_\infty\log m)^{1/2}.
\end{eqnarray*}
\end{thm}

Theorem~\ref{thm:nnls} requires the normalizations of $\hat{P}^{(r)}(\Omega)$, $1\le r\le m$, to have positive inner products. This assumption is reasonable because they are all estimates of $P(\Omega)$ and must have non-negative entries. Moreover importantly, we can directly calculate $\delta$ in practice. This condition can be replaced by the self-regularizing property of $\hat{P}^{(r)}(\Omega)$ that we present in Theorem~\ref{thm:self-regularizing} below.      

At the first glance, it may seem more natural to bound $\|\hat{P}(\Omega)- P(\Omega)\|_F$ instead of $\|\hat{P}(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F$. However, a bound for $\|\hat{P}(\Omega)- P(\Omega)\|_F$ directly follows from  \eqref{eq:nnls bound} because  
$$
\|\hat{P}(\Omega)- P(\Omega)\|_F^2 = \|\hat{P}(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F^2 + \|P(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F^2.  
$$
Note also that the error term $\|P(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F^2$ is unavoidable for all linear estimates of $P(\Omega)$ that can be formed from $\hat{P}^{(r)}$, $1\le r \le m$. Taking this into consideration, Theorem~\ref{thm:nnls} states that the proposed estimate $\hat{P}(\Omega)$ is nearly as accurate as the non-negative linear oracle $\Pi_\mathcal{C}\Pi_\mathcal{L} P(\Omega)$, where the accuracy is measured by the Frobenius norm of the deviation from the linear oracle $\Pi_\mathcal{L} P(\Omega)$. The extra error term $\varepsilon$ can be at most of the order $\log m$, although it would grow at a much slower rate if entries of $P$ and $\hat{P}^{(r)}$ are of similar orders and the network is relatively sparse.     

Similar to the discussion of the EW estimate following Theorem~\ref{thm:exp weights}, we can remove the dependence on $\Omega$ from the left-hand side of \eqref{eq:nnls bound} by applying Theorem~\ref{thm:nnls} using both $\Omega$ and $\Omega^c$ to obtain two different estimates, and then combining them to get the final estimate.     

As a consequence of Theorem~\ref{thm:nnls}, the next corollary shows that the NNLS estimate can be strictly more accurate than the OLS estimate $\Pi_\mathcal{L} A(\Omega)$, especially when $m$ is large (a typical scenario in model aggregation).  

\begin{coro}[Comparison of NNLS and OLS estimates]\label{cor:comparison}
Consider the setting in Theorem~\ref{thm:nnls} and denote 
$$\rho = \big(1-\|P(\Omega)\|_\infty\big)^2\cdot\min_{(i,j)\in\Omega} P_{ij}^2, \quad \Delta = \|\Pi_\mathcal{L}A(\Omega)-\Pi_\mathcal{L}P(\Omega)\|_F - \|\hat{P}(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F.$$ 
Assume $m \ge C\|P(\Omega)\|_\infty\rho^{-2}\log n$ for some sufficiently large constant $C>0$. Then with high probability,
\begin{equation}\label{eq:Delta bound}
\Delta \ge \frac{m^{1/2}\rho^{1/4}}{2} -C\delta^{-1/2} \max_{1\le r \le m}\frac{\|\hat{P}^{(r)}(\Omega)\|_\infty}{\|\hat{P}^{(r)}(\Omega)\|_F}\cdot\log m- \|\Pi_\mathcal{C}\Pi_\mathcal{L} P(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F. 
\end{equation} 
\end{coro}

Note that $\Delta$ is the difference between the errors incurred by the linear estimate $\Pi_\mathcal{L}A(\Omega)$ and the non-negative linear estimate $\hat{P}(\Omega)$, and $\|\Pi_\mathcal{C}\Pi_\mathcal{L} P(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F$ is the distance from the linear oracle $\Pi_\mathcal{C}P(\Omega)$ to the cone $\mathcal{C}$. To illustrate the result of Corollary~\ref{cor:comparison}, consider the setting when entries of $P$ are of the same order $d/n$, where $d$ is  the average degree. Then the assumption on $m$ is $m\ge Cd^{-1}n\log n$ and the first term on the right-hand side of \eqref{eq:Delta bound} is of order $(md/n)^{1/2}$. Therefore,
$$
\Delta \gtrsim \left(\frac{md}{n}\right)^{1/2} - \log m -  \|\Pi_\mathcal{C}\Pi_\mathcal{L} P(\Omega)-\Pi_\mathcal{L} P(\Omega)\|_F.   
$$
When $m$ is large and there exists at least a reasonably accurate estimate $\hat{P}^{(r)}(\Omega)$, the last term on the right-hand side is small, so $\Delta$ can grow as fast as $(md/n)^{1/2}-\log m$. This theoretical prediction is further supported by our empirical evidence in Section~\ref{sec:simulation}.

Finally, we can replace the assumption \eqref{eq:correlated assumption} in Theorem~\ref{thm:nnls} with the following assumption on $\hat{P}^{(r)}(\Omega)$, $1\le r\le m$, known as the self-regularizing property \cite{Slawski.NNLS.2011}. Denote by $\Sigma\in\mathbb{R}^{m\times m}$ the matrix with entries $\Sigma_{rs}=\langle \hat{P}^{(r)}(\Omega), \hat{P}^{(s)}(\Omega)\rangle$ and $\|\Sigma\|_\infty=\max_{1\le r,s\le m}|\Sigma_{rs}|$. We say that $\Sigma$ satisfies the self-regularizing property if there exists $\kappa>0$ such that for all $\beta\ge 0$, 
\begin{eqnarray}\label{eq:self-reg}
\beta^T\Sigma\beta \ge \kappa\|\Sigma\|_\infty\|\beta\|_1^2.
\end{eqnarray}

\begin{thm}[Non-negative least square estimate, self-regularization]\label{thm:self-regularizing}
Consider the setting of Theorem~\ref{thm:nnls} with condition \eqref{eq:correlated assumption} replaced by the self-regularizing property \eqref{eq:self-reg}. Then there exists a constant $C>0$ such that with high probability,
\begin{eqnarray*}
\|\hat{P}(\Omega)-\Pi_\mathcal{L}P(\Omega)\|^2 \le C\kappa^{-1}\left(\frac{\Phi^2\log^2m}{\|\Sigma\|_\infty} +\Phi\|\beta^*\|_1\log m\right),
\end{eqnarray*}
where $\Phi = \|\hat{P}^{(r)}(\Omega)\|_\infty + \|P(\Omega)\|_\infty^{1/2}\|\hat{P}^{(r)}(\Omega)\|_F$.
\end{thm}


